On Measuring Intrinsic Causal Attributions in Deep Neural Networks

Quantifying the causal influence of input features within neural networks has become a topic of increasing interest. Existing approaches typically assess direct, indirect, and total causal effects. This work treats NNs as structural causal models (SCMs) and extends our focus to include intrinsic causal contributions (ICC). We propose an identifiable generative post-hoc framework for quantifying ICC. We also draw a relationship between ICC and Sobol' indices. Our experiments on synthetic and real-world datasets demonstrate that ICC generates more intuitive and reliable explanations compared to existing global explanation techniques.

==> Images/autompg.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate1869726}{RGB}{186,97,26}
\definecolor{darkgoldenrod19413532}{RGB}{194,135,32}
\definecolor{darkkhaki21220474}{RGB}{212,204,74}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{darkslategray66}{RGB}{66,66,66}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightslategray148}{RGB}{148,148,148}
\definecolor{pink241184224}{RGB}{241,184,224}
\definecolor{rosybrown188146110}{RGB}{188,146,110}
\definecolor{rosybrown193130181}{RGB}{193,130,181}
\definecolor{seagreen21138106}{RGB}{21,138,106}
\definecolor{teal23108155}{RGB}{23,108,155}
\tikzstyle{every node}=[font=\scriptsize]
\begin{axis}[
width=\figwidth,
height=\figheight,
axis line style={lightgray204},
tick align=outside,
unbounded coords=jump,
x grid style={lightgray204},
% xlabel=\textcolor{darkslategray38}{Feature},
xmajorticks=True,
xmin=-0.5, xmax=4.5,
xtick style={color=darkslategray38},
xtick={0,1,2,3,4},
xticklabels={\fontsize{0.01pt}{0.01pt}\selectfont{cylinders},\tiny{displacement},\tiny{horsepower},\tiny{weight},\tiny{acceleration}},
% xticklabel style={rotate=45},
% y grid style={lightgray204},
% ylabel=\textcolor{darkslategray38}{Explanation},
ymajorgrids,
ymajorticks=True,
ymin=0, ymax=0.9,
ytick style={color=darkslategray38}
]
\draw[draw=white,fill=teal23108155] (axis cs:-0.4,0) rectangle (axis cs:-0.311111111111111,0.0381652781492945);
% \addlegendimage{ybar,ybar legend,draw=white,fill=teal23108155}
% \addlegendentry{Integrated Gradient}

\draw[draw=white,fill=teal23108155] (axis cs:0.6,0) rectangle (axis cs:0.688888888888889,0.0545510927635415);
\draw[draw=white,fill=teal23108155] (axis cs:1.6,0) rectangle (axis cs:1.68888888888889,0.408337243445146);
\draw[draw=white,fill=teal23108155] (axis cs:2.6,0) rectangle (axis cs:2.68888888888889,0.362734288869812);
\draw[draw=white,fill=teal23108155] (axis cs:3.6,0) rectangle (axis cs:3.68888888888889,0.136212096772205);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:-0.311111111111111,0) rectangle (axis cs:-0.222222222222222,0.149423020333803);
% \addlegendimage{ybar,ybar legend,draw=white,fill=darkgoldenrod19413532}
% \addlegendentry{Gradient * Input}

\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:0.688888888888889,0) rectangle (axis cs:0.777777777777778,0.114399878894968);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:1.68888888888889,0) rectangle (axis cs:1.77777777777778,0.368616799923888);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:2.68888888888889,0) rectangle (axis cs:2.77777777777778,0.360144947412793);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:3.68888888888889,0) rectangle (axis cs:3.77777777777778,0.00741535343454853);
\draw[draw=white,fill=seagreen21138106] (axis cs:-0.222222222222222,0) rectangle (axis cs:-0.133333333333333,0.106368791632689);
% \addlegendimage{ybar,ybar legend,draw=white,fill=seagreen21138106}
% \addlegendentry{Smooth Grad}

\draw[draw=white,fill=seagreen21138106] (axis cs:0.777777777777778,0) rectangle (axis cs:0.866666666666667,0.0296684548183471);
\draw[draw=white,fill=seagreen21138106] (axis cs:1.77777777777778,0) rectangle (axis cs:1.86666666666667,0.429441606996909);
\draw[draw=white,fill=seagreen21138106] (axis cs:2.77777777777778,0) rectangle (axis cs:2.86666666666667,0.395533262848228);
\draw[draw=white,fill=seagreen21138106] (axis cs:3.77777777777778,0) rectangle (axis cs:3.86666666666667,0.0389878837038257);
\draw[draw=white,fill=chocolate1869726] (axis cs:-0.133333333333333,0) rectangle (axis cs:-0.0444444444444445,0.0381191206569899);
% \addlegendimage{ybar,ybar legend,draw=white,fill=chocolate1869726}
% \addlegendentry{SHAP}

\draw[draw=white,fill=chocolate1869726] (axis cs:0.866666666666667,0) rectangle (axis cs:0.955555555555556,0.134951090350285);
\draw[draw=white,fill=chocolate1869726] (axis cs:1.86666666666667,0) rectangle (axis cs:1.95555555555556,0.375448095045041);
\draw[draw=white,fill=chocolate1869726] (axis cs:2.86666666666667,0) rectangle (axis cs:2.95555555555556,0.446719441139507);
\draw[draw=white,fill=chocolate1869726] (axis cs:3.86666666666667,0) rectangle (axis cs:3.95555555555556,0.00476225280817656);
\draw[draw=white,fill=rosybrown193130181] (axis cs:-0.0444444444444444,0) rectangle (axis cs:0.0444444444444444,0.0297187885318768);
% \addlegendimage{ybar,ybar legend,draw=white,fill=rosybrown193130181}
% \addlegendentry{LIME}

\draw[draw=white,fill=rosybrown193130181] (axis cs:0.955555555555556,0) rectangle (axis cs:1.04444444444444,0.0587436310245483);
\draw[draw=white,fill=rosybrown193130181] (axis cs:1.95555555555556,0) rectangle (axis cs:2.04444444444444,0.412235252104965);
\draw[draw=white,fill=rosybrown193130181] (axis cs:2.95555555555556,0) rectangle (axis cs:3.04444444444444,0.452877047139015);
\draw[draw=white,fill=rosybrown193130181] (axis cs:3.95555555555556,0) rectangle (axis cs:4.04444444444444,0.0464252811995947);
\draw[draw=white,fill=rosybrown188146110] (axis cs:0.0444444444444445,0) rectangle (axis cs:0.133333333333333,0.0122658537453014);
% \addlegendimage{ybar,ybar legend,draw=white,fill=rosybrown188146110}
% \addlegendentry{SP LIME}

\draw[draw=white,fill=rosybrown188146110] (axis cs:1.04444444444444,0) rectangle (axis cs:1.13333333333333,0.0494172461740699);
\draw[draw=white,fill=rosybrown188146110] (axis cs:2.04444444444444,0) rectangle (axis cs:2.13333333333333,0.428267200864788);
\draw[draw=white,fill=rosybrown188146110] (axis cs:3.04444444444444,0) rectangle (axis cs:3.13333333333333,0.464927037233732);
\draw[draw=white,fill=rosybrown188146110] (axis cs:4.04444444444444,0) rectangle (axis cs:4.13333333333333,0.0451226619821085);
\draw[draw=white,fill=pink241184224] (axis cs:0.133333333333333,0) rectangle (axis cs:0.222222222222222,0.0804398357868195);
% \addlegendimage{ybar,ybar legend,draw=white,fill=pink241184224}
% \addlegendentry{Permutation Feature Importance}

\draw[draw=white,fill=pink241184224] (axis cs:1.13333333333333,0) rectangle (axis cs:1.22222222222222,0.0765825659036636);
\draw[draw=white,fill=pink241184224] (axis cs:2.13333333333333,0) rectangle (axis cs:2.22222222222222,0.356063306331635);
\draw[draw=white,fill=pink241184224] (axis cs:3.13333333333333,0) rectangle (axis cs:3.22222222222222,0.432721823453903);
\draw[draw=white,fill=pink241184224] (axis cs:4.13333333333333,0) rectangle (axis cs:4.22222222222222,0.0541923977434635);
\draw[draw=white,fill=lightslategray148] (axis cs:0.222222222222222,0) rectangle (axis cs:0.311111111111111,0.0151530662551522);
% \addlegendimage{ybar,ybar legend,draw=white,fill=lightslategray148}
% \addlegendentry{ICC TOPO}

\draw[draw=white,fill=lightslategray148] (axis cs:1.22222222222222,0) rectangle (axis cs:1.31111111111111,0.00252636964432895);
\draw[draw=white,fill=lightslategray148] (axis cs:2.22222222222222,0) rectangle (axis cs:2.31111111111111,0.303965896368027);
\draw[draw=white,fill=lightslategray148] (axis cs:3.22222222222222,0) rectangle (axis cs:3.31111111111111,0.41049399971962);
\draw[draw=white,fill=lightslategray148] (axis cs:4.22222222222222,0) rectangle (axis cs:4.31111111111111,0.267860651016235);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:0.311111111111111,0) rectangle (axis cs:0.4,0.0185269210487604);
% \addlegendimage{ybar,ybar legend,draw=white,fill=darkkhaki21220474}
% \addlegendentry{ICC SHAP}

\draw[draw=white,fill=darkkhaki21220474] (axis cs:1.31111111111111,0) rectangle (axis cs:1.4,0.00284009240567684);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:2.31111111111111,0) rectangle (axis cs:2.4,0.306642204523087);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:3.31111111111111,0) rectangle (axis cs:3.4,0.413593828678131);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:4.31111111111111,0) rectangle (axis cs:4.4,0.258396983146667);
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.355555555555556 nan
-0.355555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.644444444444444 nan
0.644444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.64444444444444 nan
1.64444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.64444444444444 nan
2.64444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.64444444444444 nan
3.64444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.266666666666667 nan
-0.266666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.733333333333333 nan
0.733333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.73333333333333 nan
1.73333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.73333333333333 nan
2.73333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.73333333333333 nan
3.73333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.177777777777778 nan
-0.177777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.822222222222222 nan
0.822222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.82222222222222 nan
1.82222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.82222222222222 nan
2.82222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.82222222222222 nan
3.82222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.0888888888888889 nan
-0.0888888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.911111111111111 nan
0.911111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.91111111111111 nan
1.91111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.91111111111111 nan
2.91111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.91111111111111 nan
3.91111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.0888888888888889 nan
0.0888888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.08888888888889 nan
1.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.08888888888889 nan
2.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.08888888888889 nan
3.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.08888888888889 nan
4.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.177777777777778 nan
0.177777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.17777777777778 nan
1.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.17777777777778 nan
2.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.17777777777778 nan
3.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.17777777777778 nan
4.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.266666666666667 nan
0.266666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.26666666666667 nan
1.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.26666666666667 nan
2.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.26666666666667 nan
3.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.26666666666667 nan
4.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.355555555555556 nan
0.355555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.35555555555556 nan
1.35555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.35555555555556 nan
2.35555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.35555555555556 nan
3.35555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.35555555555556 nan
4.35555555555556 nan
};
\end{axis}

\end{tikzpicture}


==> Images/compas.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate1869726}{RGB}{186,97,26}
\definecolor{darkgoldenrod19413532}{RGB}{194,135,32}
\definecolor{darkkhaki21220474}{RGB}{212,204,74}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{darkslategray66}{RGB}{66,66,66}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightslategray148}{RGB}{148,148,148}
\definecolor{pink241184224}{RGB}{241,184,224}
\definecolor{rosybrown188146110}{RGB}{188,146,110}
\definecolor{rosybrown193130181}{RGB}{193,130,181}
\definecolor{seagreen21138106}{RGB}{21,138,106}
\definecolor{teal23108155}{RGB}{23,108,155}
\tikzstyle{every node}=[font=\scriptsize]
\begin{axis}[
width=\figwidth,
height=\figheight,
axis line style={lightgray204},
tick align=outside,
unbounded coords=jump,
x grid style={lightgray204},
% xlabel=\textcolor{darkslategray38}{Feature},
xmajorticks=False,
xmin=-0.5, xmax=6.5,
xtick style={color=darkslategray38},
xtick={0,1,2,3,4,5,6},
xticklabels={age,recidivism,prior offense count,length of stay,degree of charge,gender,race},
y grid style={lightgray204},
% ylabel=\textcolor{darkslategray38}{Explanation},
ymajorgrids,
ymajorticks=True,
ymin=0, ymax=0.9,
ytick style={color=darkslategray38}
]
\draw[draw=white,fill=teal23108155] (axis cs:-0.4,0) rectangle (axis cs:-0.311111111111111,0.41482254514927);
% \addlegendimage{ybar,ybar legend,draw=white,fill=teal23108155}
% \addlegendentry{Integrated Gradient}

\draw[draw=white,fill=teal23108155] (axis cs:0.6,0) rectangle (axis cs:0.688888888888889,0.015688428813233);
\draw[draw=white,fill=teal23108155] (axis cs:1.6,0) rectangle (axis cs:1.68888888888889,0.347257664811221);
\draw[draw=white,fill=teal23108155] (axis cs:2.6,0) rectangle (axis cs:2.68888888888889,0.180064705632585);
\draw[draw=white,fill=teal23108155] (axis cs:3.6,0) rectangle (axis cs:3.68888888888889,0.00472302809411089);
\draw[draw=white,fill=teal23108155] (axis cs:4.6,0) rectangle (axis cs:4.68888888888889,0.00382433239648078);
\draw[draw=white,fill=teal23108155] (axis cs:5.6,0) rectangle (axis cs:5.68888888888889,0.033619295103099);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:-0.311111111111111,0) rectangle (axis cs:-0.222222222222222,0);
% \addlegendimage{ybar,ybar legend,draw=white,fill=darkgoldenrod19413532}
% \addlegendentry{Gradient * Input}

\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:0.688888888888889,0) rectangle (axis cs:0.777777777777778,0.118337478771814);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:1.68888888888889,0) rectangle (axis cs:1.77777777777778,0.308000099355879);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:2.68888888888889,0) rectangle (axis cs:2.77777777777778,0.0918317901132892);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:3.68888888888889,0) rectangle (axis cs:3.77777777777778,0.0994269025889146);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:4.68888888888889,0) rectangle (axis cs:4.77777777777778,0.107236440622522);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:5.68888888888889,0) rectangle (axis cs:5.77777777777778,0.275167288547581);
\draw[draw=white,fill=seagreen21138106] (axis cs:-0.222222222222222,0) rectangle (axis cs:-0.133333333333333,0.42520561576643);
% \addlegendimage{ybar,ybar legend,draw=white,fill=seagreen21138106}
% \addlegendentry{Smooth Grad}

\draw[draw=white,fill=seagreen21138106] (axis cs:0.777777777777778,0) rectangle (axis cs:0.866666666666667,0.000967877203109096);
\draw[draw=white,fill=seagreen21138106] (axis cs:1.77777777777778,0) rectangle (axis cs:1.86666666666667,0.333248506461669);
\draw[draw=white,fill=seagreen21138106] (axis cs:2.77777777777778,0) rectangle (axis cs:2.86666666666667,0.169148919986686);
\draw[draw=white,fill=seagreen21138106] (axis cs:3.77777777777778,0) rectangle (axis cs:3.86666666666667,0.0136617103221167);
\draw[draw=white,fill=seagreen21138106] (axis cs:4.77777777777778,0) rectangle (axis cs:4.86666666666667,0.0222277747983556);
\draw[draw=white,fill=seagreen21138106] (axis cs:5.77777777777778,0) rectangle (axis cs:5.86666666666667,0.0355395954616335);
\draw[draw=white,fill=chocolate1869726] (axis cs:-0.133333333333333,0) rectangle (axis cs:-0.0444444444444445,0.473081279602167);
% \addlegendimage{ybar,ybar legend,draw=white,fill=chocolate1869726}
% \addlegendentry{SHAP}

\draw[draw=white,fill=chocolate1869726] (axis cs:0.866666666666667,0) rectangle (axis cs:0.955555555555556,0.16362840935588);
\draw[draw=white,fill=chocolate1869726] (axis cs:1.86666666666667,0) rectangle (axis cs:1.95555555555556,0.00328028229121823);
\draw[draw=white,fill=chocolate1869726] (axis cs:2.86666666666667,0) rectangle (axis cs:2.95555555555556,0.029851879435097);
\draw[draw=white,fill=chocolate1869726] (axis cs:3.86666666666667,0) rectangle (axis cs:3.95555555555556,0.13832346729682);
\draw[draw=white,fill=chocolate1869726] (axis cs:4.86666666666667,0) rectangle (axis cs:4.95555555555556,0.0421171348904541);
\draw[draw=white,fill=chocolate1869726] (axis cs:5.86666666666667,0) rectangle (axis cs:5.95555555555556,0.149717547128363);
\draw[draw=white,fill=rosybrown193130181] (axis cs:-0.0444444444444444,0) rectangle (axis cs:0.0444444444444444,0.508199149671389);
% \addlegendimage{ybar,ybar legend,draw=white,fill=rosybrown193130181}
% \addlegendentry{LIME}

\draw[draw=white,fill=rosybrown193130181] (axis cs:0.955555555555556,0) rectangle (axis cs:1.04444444444444,0.0360462873347885);
\draw[draw=white,fill=rosybrown193130181] (axis cs:1.95555555555556,0) rectangle (axis cs:2.04444444444444,0.289496861588751);
\draw[draw=white,fill=rosybrown193130181] (axis cs:2.95555555555556,0) rectangle (axis cs:3.04444444444444,0.0664175561022849);
\draw[draw=white,fill=rosybrown193130181] (axis cs:3.95555555555556,0) rectangle (axis cs:4.04444444444444,0.0420613569530734);
\draw[draw=white,fill=rosybrown193130181] (axis cs:4.95555555555556,0) rectangle (axis cs:5.04444444444444,0.0104914348078336);
\draw[draw=white,fill=rosybrown193130181] (axis cs:5.95555555555556,0) rectangle (axis cs:6.04444444444444,0.0472873535418794);
\draw[draw=white,fill=rosybrown188146110] (axis cs:0.0444444444444445,0) rectangle (axis cs:0.133333333333333,0.497888639678127);
% \addlegendimage{ybar,ybar legend,draw=white,fill=rosybrown188146110}
% \addlegendentry{SP LIME}

\draw[draw=white,fill=rosybrown188146110] (axis cs:1.04444444444444,0) rectangle (axis cs:1.13333333333333,0.0427872749652088);
\draw[draw=white,fill=rosybrown188146110] (axis cs:2.04444444444444,0) rectangle (axis cs:2.13333333333333,0.290460215146443);
\draw[draw=white,fill=rosybrown188146110] (axis cs:3.04444444444444,0) rectangle (axis cs:3.13333333333333,0.0772752481195162);
\draw[draw=white,fill=rosybrown188146110] (axis cs:4.04444444444444,0) rectangle (axis cs:4.13333333333333,0.0326251329782551);
\draw[draw=white,fill=rosybrown188146110] (axis cs:5.04444444444444,0) rectangle (axis cs:5.13333333333333,0.00668313152125755);
\draw[draw=white,fill=rosybrown188146110] (axis cs:6.04444444444444,0) rectangle (axis cs:6.13333333333333,0.052280357591193);
\draw[draw=white,fill=pink241184224] (axis cs:0.133333333333333,0) rectangle (axis cs:0.222222222222222,0.321030974388123);
% \addlegendimage{ybar,ybar legend,draw=white,fill=pink241184224}
% \addlegendentry{Permutation Feature Importance}

\draw[draw=white,fill=pink241184224] (axis cs:1.13333333333333,0) rectangle (axis cs:1.22222222222222,0.0469958521425724);
\draw[draw=white,fill=pink241184224] (axis cs:2.13333333333333,0) rectangle (axis cs:2.22222222222222,0.42127314209938);
\draw[draw=white,fill=pink241184224] (axis cs:3.13333333333333,0) rectangle (axis cs:3.22222222222222,0.0869400799274445);
\draw[draw=white,fill=pink241184224] (axis cs:4.13333333333333,0) rectangle (axis cs:4.22222222222222,0.0319956056773663);
\draw[draw=white,fill=pink241184224] (axis cs:5.13333333333333,0) rectangle (axis cs:5.22222222222222,0.0225941613316536);
\draw[draw=white,fill=pink241184224] (axis cs:6.13333333333333,0) rectangle (axis cs:6.22222222222222,0.0691701918840408);
\draw[draw=white,fill=lightslategray148] (axis cs:0.222222222222222,0) rectangle (axis cs:0.311111111111111,0.31646528840065);
% \addlegendimage{ybar,ybar legend,draw=white,fill=lightslategray148}
% \addlegendentry{ICC TOPO}

\draw[draw=white,fill=lightslategray148] (axis cs:1.22222222222222,0) rectangle (axis cs:1.31111111111111,0.508557975292206);
\draw[draw=white,fill=lightslategray148] (axis cs:2.22222222222222,0) rectangle (axis cs:2.31111111111111,0.117647014558315);
\draw[draw=white,fill=lightslategray148] (axis cs:3.22222222222222,0) rectangle (axis cs:3.31111111111111,0.0111270174384117);
\draw[draw=white,fill=lightslategray148] (axis cs:4.22222222222222,0) rectangle (axis cs:4.31111111111111,0.00769776431843638);
\draw[draw=white,fill=lightslategray148] (axis cs:5.22222222222222,0) rectangle (axis cs:5.31111111111111,0.000189099577255547);
\draw[draw=white,fill=lightslategray148] (axis cs:6.22222222222222,0) rectangle (axis cs:6.31111111111111,0.0348277911543846);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:0.311111111111111,0) rectangle (axis cs:0.4,0.453807294368744);
% \addlegendimage{ybar,ybar legend,draw=white,fill=darkkhaki21220474}
% \addlegendentry{ICC SHAP}

\draw[draw=white,fill=darkkhaki21220474] (axis cs:1.31111111111111,0) rectangle (axis cs:1.4,0.301909029483795);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:2.31111111111111,0) rectangle (axis cs:2.4,0.151026725769043);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:3.31111111111111,0) rectangle (axis cs:3.4,0.0132208317518234);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:4.31111111111111,0) rectangle (axis cs:4.4,0.00910740997642279);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:5.31111111111111,0) rectangle (axis cs:5.4,0.000695095863193274);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:6.31111111111111,0) rectangle (axis cs:6.4,0.0667800754308701);
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.355555555555556 nan
-0.355555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.644444444444444 nan
0.644444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.64444444444444 nan
1.64444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.64444444444444 nan
2.64444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.64444444444444 nan
3.64444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.64444444444444 nan
4.64444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
5.64444444444444 nan
5.64444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.266666666666667 nan
-0.266666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.733333333333333 nan
0.733333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.73333333333333 nan
1.73333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.73333333333333 nan
2.73333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.73333333333333 nan
3.73333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.73333333333333 nan
4.73333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
5.73333333333333 nan
5.73333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.177777777777778 nan
-0.177777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.822222222222222 nan
0.822222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.82222222222222 nan
1.82222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.82222222222222 nan
2.82222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.82222222222222 nan
3.82222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.82222222222222 nan
4.82222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
5.82222222222222 nan
5.82222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.0888888888888889 nan
-0.0888888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.911111111111111 nan
0.911111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.91111111111111 nan
1.91111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.91111111111111 nan
2.91111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.91111111111111 nan
3.91111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.91111111111111 nan
4.91111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
5.91111111111111 nan
5.91111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3 nan
3 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4 nan
4 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
5 nan
5 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
6 nan
6 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.0888888888888889 nan
0.0888888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.08888888888889 nan
1.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.08888888888889 nan
2.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.08888888888889 nan
3.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.08888888888889 nan
4.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
5.08888888888889 nan
5.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
6.08888888888889 nan
6.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.177777777777778 nan
0.177777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.17777777777778 nan
1.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.17777777777778 nan
2.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.17777777777778 nan
3.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.17777777777778 nan
4.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
5.17777777777778 nan
5.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
6.17777777777778 nan
6.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.266666666666667 nan
0.266666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.26666666666667 nan
1.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.26666666666667 nan
2.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.26666666666667 nan
3.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.26666666666667 nan
4.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
5.26666666666667 nan
5.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
6.26666666666667 nan
6.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.355555555555556 nan
0.355555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.35555555555556 nan
1.35555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.35555555555556 nan
2.35555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
3.35555555555556 nan
3.35555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
4.35555555555556 nan
4.35555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
5.35555555555556 nan
5.35555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
6.35555555555556 nan
6.35555555555556 nan
};
\end{axis}

\end{tikzpicture}


==> Images/synthetic.tex <==
% This file was created with tikzplotlib v0.10.1.
\begin{tikzpicture}

\definecolor{chocolate1869726}{RGB}{186,97,26}
\definecolor{darkgoldenrod19413532}{RGB}{194,135,32}
\definecolor{darkkhaki21220474}{RGB}{212,204,74}
\definecolor{darkslategray38}{RGB}{38,38,38}
\definecolor{darkslategray66}{RGB}{66,66,66}
\definecolor{lightgray204}{RGB}{204,204,204}
\definecolor{lightslategray148}{RGB}{148,148,148}
\definecolor{pink241184224}{RGB}{241,184,224}
\definecolor{rosybrown188146110}{RGB}{188,146,110}
\definecolor{rosybrown193130181}{RGB}{193,130,181}
\definecolor{seagreen21138106}{RGB}{21,138,106}
\definecolor{teal23108155}{RGB}{23,108,155}
\tikzstyle{every node}=[font=\scriptsize]
\begin{axis}[
width=\figwidth,
height=\figheight,
axis line style={lightgray204},
tick align=outside,
unbounded coords=jump,
x grid style={lightgray204},
% xlabel=\textcolor{darkslategray38}{Feature},
xmajorticks=True,
xmin=-0.5, xmax=2.5,
xtick style={color=darkslategray38},
xtick={0,1,2},
xticklabels={W,Z,X},
y grid style={lightgray204},
% ylabel=\textcolor{darkslategray38}{Explanation},
ymajorgrids,
ymajorticks=True,
ymin=0, ymax=0.9,
ytick style={color=darkslategray38}
legend style={
        at={(1.05,1)},
        anchor=north west,
        font=\tiny,
        legend cell align=left
    }
    % legend entries={
    %     {IG},
    %     {ITG},
    %     {SG},
    %     {SHAP},
    %     {LIME},
    %     {SP LIME},
    %     {Permutation Feature Importanc},
    %     {ICC TOPO},
    %     {ICC SHAP}
    % }
]
\draw[draw=white,fill=teal23108155] (axis cs:-0.4,0) rectangle (axis cs:-0.311111111111111,0.00978335929781006);
% \addlegendimage{ybar,ybar legend,draw=white,fill=teal23108155}
% \addlegendentry{\textbf{\tiny{IG}}}

\draw[draw=white,fill=teal23108155] (axis cs:0.6,0) rectangle (axis cs:0.688888888888889,0.615714665958847);
\draw[draw=white,fill=teal23108155] (axis cs:1.6,0) rectangle (axis cs:1.68888888888889,0.374501974743343);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:-0.311111111111111,0) rectangle (axis cs:-0.222222222222222,0.0277655983693334);
% \addlegendimage{ybar,ybar legend,draw=white,fill=darkgoldenrod19413532}
% \addlegendentry{\tiny{\textbf{I$\times$G} }}

\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:0.688888888888889,0) rectangle (axis cs:0.777777777777778,0.599263438484965);
\draw[draw=white,fill=darkgoldenrod19413532] (axis cs:1.68888888888889,0) rectangle (axis cs:1.77777777777778,0.372970963145701);
\draw[draw=white,fill=seagreen21138106] (axis cs:-0.222222222222222,0) rectangle (axis cs:-0.133333333333333,0.00368323630295408);
% \addlegendimage{ybar,ybar legend,draw=white,fill=seagreen21138106}
% \addlegendentry{\tiny{\textbf{SG}}}

\draw[draw=white,fill=seagreen21138106] (axis cs:0.777777777777778,0) rectangle (axis cs:0.866666666666667,0.569648370924546);
\draw[draw=white,fill=seagreen21138106] (axis cs:1.77777777777778,0) rectangle (axis cs:1.86666666666667,0.4266683927725);
\draw[draw=white,fill=chocolate1869726] (axis cs:-0.133333333333333,0) rectangle (axis cs:-0.0444444444444445,0.0462342949393222);
% \addlegendimage{ybar,ybar legend,draw=white,fill=chocolate1869726}
% \addlegendentry{\tiny{\textbf{SHAP}}}

\draw[draw=white,fill=chocolate1869726] (axis cs:0.866666666666667,0) rectangle (axis cs:0.955555555555556,0.671552317584217);
\draw[draw=white,fill=chocolate1869726] (axis cs:1.86666666666667,0) rectangle (axis cs:1.95555555555556,0.282213387476461);
\draw[draw=white,fill=rosybrown193130181] (axis cs:-0.0444444444444444,0) rectangle (axis cs:0.0444444444444444,0.0494674066578089);
% \addlegendimage{ybar,ybar legend,draw=white,fill=rosybrown193130181}
% \addlegendentry{\tiny{\textbf{LIME}}}

\draw[draw=white,fill=rosybrown193130181] (axis cs:0.955555555555556,0) rectangle (axis cs:1.04444444444444,0.508024887901937);
\draw[draw=white,fill=rosybrown193130181] (axis cs:1.95555555555556,0) rectangle (axis cs:2.04444444444444,0.442507705440254);
\draw[draw=white,fill=rosybrown188146110] (axis cs:0.0444444444444445,0) rectangle (axis cs:0.133333333333333,0.0859830216264728);
% \addlegendimage{ybar,ybar legend,draw=white,fill=rosybrown188146110}
% \addlegendentry{\tiny{\textbf{SP-LIME}}}

\draw[draw=white,fill=rosybrown188146110] (axis cs:1.04444444444444,0) rectangle (axis cs:1.13333333333333,0.53598263683838);
\draw[draw=white,fill=rosybrown188146110] (axis cs:2.04444444444444,0) rectangle (axis cs:2.13333333333333,0.378034341535148);
\draw[draw=white,fill=pink241184224] (axis cs:0.133333333333333,0) rectangle (axis cs:0.222222222222222,0.14023169875145);
% \addlegendimage{ybar,ybar legend,draw=white,fill=pink241184224}
% \addlegendentry{\tiny{\textbf{PFI}}}

\draw[draw=white,fill=pink241184224] (axis cs:1.13333333333333,0) rectangle (axis cs:1.22222222222222,0.455315917730331);
\draw[draw=white,fill=pink241184224] (axis cs:2.13333333333333,0) rectangle (axis cs:2.22222222222222,0.404452413320541);
\draw[draw=white,fill=lightslategray148] (axis cs:0.222222222222222,0) rectangle (axis cs:0.311111111111111,0.00744294514879584);
% \addlegendimage{ybar,ybar legend,draw=white,fill=lightslategray148}
% \addlegendentry{\tiny{$\mathbf{ICC^{\text{To}}}$}}

\draw[draw=white,fill=lightslategray148] (axis cs:1.22222222222222,0) rectangle (axis cs:1.31111111111111,0.815784633159637);
\draw[draw=white,fill=lightslategray148] (axis cs:2.22222222222222,0) rectangle (axis cs:2.31111111111111,0.176772400736809);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:0.311111111111111,0) rectangle (axis cs:0.4,0.013973843306303);
% \addlegendimage{ybar,ybar legend,draw=white,fill=darkkhaki21220474}
% \addlegendentry{\tiny{$\mathbf{ICC^{\text{Sh}}}$}}

\draw[draw=white,fill=darkkhaki21220474] (axis cs:1.31111111111111,0) rectangle (axis cs:1.4,0.832258939743042);
\draw[draw=white,fill=darkkhaki21220474] (axis cs:2.31111111111111,0) rectangle (axis cs:2.4,0.153767213225365);
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.355555555555556 nan
-0.355555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.644444444444444 nan
0.644444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.64444444444444 nan
1.64444444444444 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.266666666666667 nan
-0.266666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.733333333333333 nan
0.733333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.73333333333333 nan
1.73333333333333 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.177777777777778 nan
-0.177777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.822222222222222 nan
0.822222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.82222222222222 nan
1.82222222222222 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
-0.0888888888888889 nan
-0.0888888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.911111111111111 nan
0.911111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.91111111111111 nan
1.91111111111111 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0 nan
0 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1 nan
1 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2 nan
2 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.0888888888888889 nan
0.0888888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.08888888888889 nan
1.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.08888888888889 nan
2.08888888888889 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.177777777777778 nan
0.177777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.17777777777778 nan
1.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.17777777777778 nan
2.17777777777778 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.266666666666667 nan
0.266666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.26666666666667 nan
1.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.26666666666667 nan
2.26666666666667 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
0.355555555555556 nan
0.355555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
1.35555555555556 nan
1.35555555555556 nan
};
\addplot [line width=1.08pt, darkslategray66]
table {%
2.35555555555556 nan
2.35555555555556 nan
};
\end{axis}

\end{tikzpicture}

